Self-supervised Visual Attribute Learning for Fashion Compatibility

Many self-supervised learning (SSL) methods have been successful in learning semantically meaningful visual representations by solving pretext tasks. However, prior work in SSL focuses on tasks like object recognition or detection, which aim to learn object shapes and assume that the features should be invariant to concepts like colors and textures. Thus, these SSL methods perform poorly on downstream tasks where these concepts provide critical information. In this paper, we present an SSL framework that enables us to learn color and texture-aware features without requiring any labels during training. Our approach consists of three self-supervised tasks designed to capture different concepts that are neglected in prior work that we can select from depending on the needs of our downstream tasks. Our tasks include learning to predict color histograms and discriminate shapeless local patches and textures from each instance. We evaluate our approach on fashion compatibility using Polyvore Outfits and In-Shop Clothing Retrieval using Deepfashion, improving upon prior SSL methods by 9.5-16%, and even outperforming some supervised approaches on Polyvore Outfits despite using no labels. We also show that our approach can be used for transfer learning, demonstrating that we can train on one dataset while achieving high performance on a different dataset.

==> figure/fig_supp_tsne_ID.tex <==
\begin{figure*}[h]
	\centering
% 	\begin{subfigure}[t]{1.0\textwidth}
    \includegraphics[width=\linewidth]{imgs/supp_tsne_ID.jpg}
    \caption{t-SNE visualization of features from Instance Discrimination~\cite{wu2018unsupervised} without shapeless local patch.}
	\label{fig:supp_tsne_id}
	\vspace{-4mm}
\end{figure*}


==> figure/fig_supp_tsne_RGB.tex <==
\begin{figure*}[h]
	\centering
% 	\begin{subfigure}[t]{1.0\textwidth}
    % \hspace{-1.0in}
    \includegraphics[width=\linewidth]{imgs/supp_tsne_RGB.jpg}
    \caption{t-SNE visualization of features from predicting RGB histrograms (ours).}
	\label{fig:supp_tsne_rgb}
	\vspace{-4mm}
\end{figure*}


==> figure/fig_supp_tsne_bilinear.tex <==
\begin{figure*}[t]
	\centering
% 	\begin{subfigure}[t]{1.0\textwidth}
    % \hspace{-1.0in}
    \includegraphics[width=\linewidth]{imgs/supp_tsne_bilinear.jpg}
    \caption{t-SNE visualization of features from texture discrimination (ours).}
	\label{fig:supp_tsne_bilinear}
	\vspace{-4mm}
\end{figure*}


==> figure/fig_supp_tsne_imagenet.tex <==
\begin{figure*}[h]
	\centering
% 	\begin{subfigure}[t]{1.0\textwidth}
    % \hspace{-1.2in}
    \includegraphics[width=\linewidth]{imgs/sup_tsne_imgenet.jpg}
    \caption{t-SNE visualization of features from the ImageNet pret-rained model.}
	\label{fig:supp_tsne_imagenet} 
	\vspace{-4mm}
\end{figure*}


==> figure/fig_supp_tsne_ours.tex <==
\begin{figure*}[h]
	\centering
% 	\begin{subfigure}[t]{1.0\textwidth}
    % \hspace{-1.2in}
    \includegraphics[width=1.0\linewidth]{imgs/supp_tsne_ours.jpg}
    \caption{t-SNE visualization of features from S-VAL (ours).}
	\label{fig:supp_tsne_ours} 
	\vspace{-4mm}
\end{figure*}


==> figure/fig_supp_tsne_slpd.tex <==
\begin{figure*}[h]
	\centering
% 	\begin{subfigure}[t]{1.0\textwidth}
    % \hspace{-1.0in}
    \includegraphics[width=\linewidth]{imgs/supp_tsne_slpd.jpg}
    \caption{t-SNE visualization of features from SLPD (ours).}
	\label{fig:supp_tsne_slpd}
	\vspace{-4mm}
\end{figure*}


==> figure/fig_supp_tsne_supervised.tex <==
\begin{figure*}[h]
	\centering
% 	\begin{subfigure}[t]{1.0\textwidth}
    % \hspace{-1.0in}
    \includegraphics[width=\linewidth]{imgs/supp_tsne_supervised.jpg}
    \caption{t-SNE visualization of features from the Siamese Network~\cite{vasileva2018learning} trained on compatibility labels.}
	\label{fig:supp_tsne_sup}
	\vspace{-4mm}
\end{figure*}


==> table/supp_table_others.tex <==
% \begin{SCtable}
% % \centering
% \caption{Cross dataset experiments. We train a model on the Fashion-Gen dataset and test it on the Polyvore dataset. We report the performances of (a)  self-supervised learning baselines and (b) ours. Our method is able to generalize across different datasets.}

% % \begin{subtable}[t]{0.5\textwidth}
% % \caption{Cross Dataset Evaluation}
% \begin{tabular}{|ll|c|c|}
% \hline
%  & & \multicolumn{2}{c|}{Fashion-Gen $\rightarrow$ Polyvore} \\
%  \hline
%     &Method & Comp. AUC & FITB acc.   \\
% \hline
% \hline
% (a)   & ID~\cite{wu2018unsupervised} & 0.71 & 45.5 \\
%   &    Local Agg.~\cite{zhuang2019local} & 0.73 & 46.5\\
%     \hline
% (b)&    RGB & 0.76 & 48.1  \\ 
%     % SLPD & 0.80 & 52.6 \\
%     % TD & 0.76 & 49.9 \\
%  &   RGB+SLPD & 0.81 & 54.0 \\
%   &  RGB+SLPD+TD & \textbf{0.82} & \textbf{54.2} \\
% % \hline
% \hline
% \end{tabular}
% % \end{subtable}

% \label{exp:tab_1}
% \end{SCtable}



\begin{table}[h]
\centering

\resizebox{0.49\textwidth}{!}{\begin{tabular}{|l|c|c|c|}
\hline
 & \multicolumn{2}{c|}{Polyvore Outfits} & Capsule \\
\hline
    Method & Comp. AUC & FITB acc. & Comp. AUC  \\
\hline
% \hline
    RGB & 0.77 $\pm$ 0 & 47.2 $\pm$ 0.23 & 23.3 $\pm$ 0.1\\ 
    SLPD & 0.83 $\pm$ 0 & 54.6 $\pm$ 0.52 & 27.7 $\pm$ 0.25\\
    TD & 0.77 $\pm$ 0  & 50.3 $\pm$ 0.36 & 25.2 $\pm$ 0.37 \\
    RGB+SLPD & 0.83  $\pm$ 0 & 55.4 $\pm$ 0.35 & 27.7 $\pm$0.15 \\
    RGB+SLPD+TD & 0.84 $\pm$ 0 & 55.8 $\pm$ 0.15 & 27.9 $\pm$ 0.15 \\
% \hline
\hline
\end{tabular}}
\caption{Standard deviation over three runs on Polyvore Outfits~\cite{vasileva2018learning} for the fashion compatibility task.}
\label{exp:supp_std}
\vspace{-4mm}
\end{table}

==> table/table_polyvore.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|ll|c|c|c|c|}
\hline
 & &\multirow{2}{*}{Label?}  & \multicolumn{2}{c|}{Polyvore Outfits} & Capsule  \\
 \cline{4-6}
& Method & & Comp. AUC  &  FITB acc. & Comp. AUC \\
\hline
\hline
(a) & Type-Aware Network~\cite{vasileva2018learning} & Comp. &  0.86 & 55.3 & -\\
    & SCE-Net~\cite{tan2019learning} & Comp. & 0.91 & 61.6 & -  \\
    % & SiameseNet (our implementation) & 0.92 & 63.0 & 47.0 \\
    & SiameseNet~\cite{vasileva2018learning} & Comp. & 0.81 & 52.9 & - \\
    & Attribute  & Attribute & 0.73  & 46.3  & 25.0 \\
    \hline
    \hline
(b) & ImageNet pre-trained & \xmark & 0.66 & 39.1  & 21.1  \\
    & Capsule Network~\cite{hsiao2018creating} & \xmark  & - & -  & 19.9  \\
    & AutoEncoder~\cite{hinton1994autoencoders} & \xmark  & 0.58 & 34.0  & 19.8  \\
    & Colorization~\cite{zhang2016colorful} & \xmark  &  0.63 & 34.1 & 18.6  \\
    & Jigsaw~\cite{noroozi2016unsupervised} & \xmark  & 0.52 & 27.9  & 18.6  \\
    & Rotation~\cite{gidaris2018unsupervised} & \xmark  & 0.53 & 29.4  & 18.5  \\
    & ID w/ color distortion \cite{wu2018unsupervised} & \xmark  & 0.57  & 30.8  & 18.9  \\
    & ID w/o color distortion & \xmark  & 0.74 & 45.9  & 23.3  \\
    & Local Agg. w/ color distortion \cite{zhuang2019local} & \xmark & 0.56  & 30.4  & 19.1  \\
    & Local Agg. w/o color distortion & \xmark  & 0.74 & 46.3  & 24.0   \\
    \hline
(c) & Predicting RGB histogram (RGB) & \xmark  & 0.77 & 47.3    &  23.4   \\
    & Shapeless Local Patch Disc. (SLPD) & \xmark  & 0.82 & 54.0 &  27.4   \\
    & Texture Disc (TD) & \xmark & 0.76 & 49.9    &  25.6   \\
    & RGB + SLPD & \xmark  & 0.83 & 55.1    &  27.7   \\
    & RGB + SLPD + TD & \xmark  & \textbf{0.84} & \textbf{55.8}    &  \textbf{28.0}   \\
% \hline
\hline
\end{tabular}
\caption{Comparison of (a) supervised models with compatibility or attribute labels and (b,c) unsupervised models on the Polyvore Outfits~\cite{vasileva2018learning} and Capsule~\cite{hsiao2018creating} datasets. \textit{All methods are initiailized with ImageNet pre-trained weight and finetuned on Polyvore Outfits.} We report the performance of existing self-supervised learning baselines in (b) and our proposed components in (c).}
\label{exp:tab_polyvore}
\end{table*}


% \begin{table}[]
% \centering
% \caption{Performance comparison on the Polyvore~\cite{vasileva2018learning} and Capsule~\cite{hsiao2018creating} datasets. (a) reports the performances of supervised or weakly-supervised model trained on item compatibility or attribute labels, (b) reports the performances the prior self-supervised learning, and (c) reports the performances of our proposed components.}
% \begin{tabular}{|ll|c|c|c|}
% \hline
%  & & \multicolumn{2}{c|}{Polyvore Outfits} & Capsule Ward.  \\
%  \hline
% & Method &  FITB acc. &  Compat. AUC & Compat. AUC \\
% \hline
% \hline
%  (a)& \textbf{Supervised Learning} & & &\\
% %  \hline
%  & Type-Aware Embedding Network~\cite{vasileva2018learning} & 0.86 & 55.3 & -\\
%     & SCE-Net~\cite{tan2019learning} & 0.91 & 61.6 & -  \\
%     % & SiameseNet (our implementation) & 0.92 & 63.0 & 47.0 \\
%     & Attribute (weakly-supervised) & 0.73  & 46.3  & 25.0 \\
%     \hline
%     \hline
% (b)  &
%      & ImageNet pre-trained & 0.66 & 39.1  & 21.1  \\
%     & Capsule Network~\cite{hsiao2018creating} & - & -  & 19.9  \\
%     & AutoEncoder~\cite{hinton1994autoencoders} & 0.58 & 34.0  & 19.8  \\
%     & Colorization~\cite{zhang2016colorful} &  0.63 & 34.1 & 18.6  \\
%     & Jigsaw~\cite{noroozi2016unsupervised} & 0.52 & 27.9  & 18.6  \\
%     & Rotation~\cite{gidaris2018unsupervised} & 0.53 & 29.4  & 18.5  \\
%     & ID w/ color distortion \cite{wu2018unsupervised} & 0.57  & 30.8  & 18.9  \\
%     & ID w/o color distortion & 0.74 & 45.9  & 23.3  \\
%     & Local Aggregation w/ color distortion \cite{zhuang2019local} & 0.56  & 30.4  & 19.1  \\
%     & Local Aggregation w/o color distortion  & 0.74 & 46.3  & 24.0   \\
%     % \hline
% (c) & Predicting RGB histogram (RGB) & 0.77 & 47.6    &  23.4   \\
%     & Shapeless Local Patch Disc. (SLPD) & 0.82 & 54.0 &  27.4   \\
%     & Texture Disc (TD) & 0.76 & 49.9    &  25.6   \\
%     & RGB + SLPD & 0.83 & 55.1    &  27.7   \\
%     & RGB + SLPD + TD & \textbf{0.84} & \textbf{55.8}    &  \textbf{28.0}   \\
% % \hline
% \hline
% \end{tabular}

% \label{exp:tab_polyvore}
% \end{table}
